Scalable Decision-Making in Stochastic Environments through Learned Temporal Abstraction

Sequential decision-making in high-dimensional continuous action spaces, particularly in stochastic environments, faces significant computational challenges. We explore this challenge in the traditional offline RL setting, where an agent must learn how to make decisions based on data collected through a stochastic behavior policy. We present Latent Macro Action Planner (L-MAP), which addresses this challenge by learning a set of temporally extended macro-actions through a state-conditional Vector Quantized Variational Autoencoder (VQ-VAE), effectively reducing action dimensionality. L-MAP employs a (separate) learned prior model that acts as a latent transition model and allows efficient sampling of plausible actions. During planning, our approach accounts for stochasticity in both the environment and the behavior policy by using Monte Carlo tree search (MCTS). In offline RL settings, including stochastic continuous control tasks, L-MAP efficiently searches over discrete latent actions to yield high expected returns. Empirical results demonstrate that L-MAP maintains low decision latency despite increased action dimensionality. Notably, across tasks ranging from continuous control with inherently stochastic dynamics to high-dimensional robotic hand manipulation, L-MAP significantly outperforms existing model-based methods and performs on-par with strong model-free actor-critic baselines, highlighting the effectiveness of the proposed approach in planning in complex and stochastic environments with high-dimensional action spaces.

==> main/algorithm/progressive_widening.tex <==
\begin{algorithm}
\caption{Progressive Widening for Node Expansion}
\begin{algorithmic}[1]
\Procedure{Sample}{$s, z$}
    \State $N \gets \text{num\_visits}[s, z]$
    \If{$\text{num\_children}[s, z] < kN^\alpha$}
        \State $z' \sim T(s, z)$ \Comment{Sample new latent code from transition model}
        \If{$z' \notin \text{children}[s, z]$}
            \State $\text{children}[s, z].\text{add}(z')$
        \EndIf
        \State \Return $z'$
    \Else
        \State \Return $\text{sample}(\text{children}[s, z])$
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> main/table/ablation_study_P-UCB.tex <==
\begin{table}[htbp]
\centering
\caption{UCB vs P-UCB}
%\label{tab:results}
\begin{adjustbox}{width=0.85\textwidth}
\begin{tabular}{llcc}
\toprule
\textbf{Dataset Type} & \textbf{Environment} & \textbf{Model-Based (\map)} & \textbf{Model-Based (\map+P-UCB)} & \textbf{ (\map+modified P-UCB)}\\
\midrule
Medium-Expert-Mod  & Hopper     & 106.11 $\pm$ 2.16    &  106.88 $\pm$ 2.13\\
Medium-Expert-Mod  & Walker2D   & \textbf{93.43 $\pm$ 1.41} & 90.04 $\pm$ 1.59 \\
Medium-Mod         & Hopper     & 55.07 $\pm$ 3.06    &  49.10 $\pm$ 2.93 \\
Medium-Mod         & Walker2D   & 52.94 $\pm$ 1.57    &  49.32 $\pm$ 2.19\\
Medium-Replay-Mod  & Hopper     & \textbf{52.30 $\pm$ 2.65} & 45.27 $\pm$ 2.66 \\ 
Medium-Replay-Mod  & Walker2D   & \textbf{51.44 $\pm$ 1.65} &  47.67 $\pm$ 1.70 \\
Medium-Expert-High & Hopper     & \textbf{66.93 $\pm$ 3.46} &  65.56 $\pm$ 3.74\\
Medium-Expert-High & Walker2D   & \textbf{97.18 $\pm$ 2.08} &  97.18 $\pm$ 2.08\\
Medium-High        & Hopper     & \textbf{55.32 $\pm$ 3.56} & 50.40 $\pm$ 3.46\\
Medium-High        & Walker2D   & \textbf{68.87 $\pm$ 2.21} &   61.36 $\pm$ 2.92\\
Medium-Replay-High & Hopper     & 58.05 $\pm$ 3.36    & 57.82 $\pm$ 3.47 \\
Medium-Replay-High & Walker2D   & \textbf{65.87 $\pm$ 3.07} & 66.05 $\pm$ 2.79\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
%68.70


==> main/table/ablation_study_latent_step.tex <==
\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
%\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{Step=1} & \textbf{Step=3} & \textbf{Step=5} \\
\midrule
Medium-Expert-High & Hopper      & 69.23 $\pm$ 4.08  & 66.93 ± 3.46 & 61.19 $\pm$ 3.80 \\
Medium-Expert-High & Walker2D    & 93.41 $\pm$ 2.30 & 97.18 ± 2.08*  &  99.02 $\pm$ 2.63\\
\midrule
Medium-High        & Hopper      & 54.76 $\pm$ 3.10  &  55.32 ± 3.56* &  46.52 $\pm$ 3.27\\
Medium-High        & Walker2D    & 66.72 $\pm$ 2.33  & 68.87 ± 2.21*  &   63.94 $\pm$ 2.55\\
\midrule
Medium-Replay-High & Hopper      & 42.57 $\pm$ 2.62  &  58.05 ± 3.36  & 54.03 $\pm$ 3.40 \\
Medium-Replay-High & Walker2D    & 59.63 $\pm$ 3.04  &  65.87 ± 3.07* &  62.72 $\pm$ 3.47\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

%64.39; 68.70; 64.57

==> main/table/ablation_study_mcts_iterations.tex <==
\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
%\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{Iteration=50} & \textbf{Horizon=100} & \textbf{Iteration=10} \\
\midrule
Medium-Expert-High & Hopper      &  62.40 +/- 3.73 & 66.93 ± 3.46 &   56.32 +/- 3.24\\
Medium-Expert-High & Walker2D    &  97.67 +/- 2.56& 97.18 ± 2.0  &  94.53 +/- 2.24\\
\midrule
Medium-High        & Hopper      & 48.44 +/- 3.23  &  55.32 ± 3.56 &  47.48 +/- 3.20\\
Medium-High        & Walker2D    &  65.98 +/- 2.41 & 68.87 ± 2.21  & 66.14 +/- 2.41\\
\midrule
Medium-Replay-High & Hopper      &  52.75 +/- 3.09 &  62.49 ± 3.65 & 47.16 +/- 2.89\\
Medium-Replay-High & Walker2D    &  64.30 +/- 3.10  & 65.87 ± 3.07  & 52.41 +/- 3.12\\

%65.26&68.23&60.67
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> main/table/ablation_study_parallel_expand.tex <==
\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
%\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{$no parallel$} & \textbf{$\alpha$=1} \\
\midrule
Medium-Expert-High & Hopper      &   & 63.92 +/- 3.45 &  \\
Medium-Expert-High & Walker2D    &   & 97.00 +/- 2.67 &  \\
\midrule
Medium-High        & Hopper      &   & 52.47 +/- 3.57 &  \\
Medium-High        & Walker2D    &   & 62.03 +/- 2.78 &  \\
\midrule
Medium-Replay-High & Hopper      &   & 51.42 +/- 3.22 &  \\
Medium-Replay-High & Walker2D    &   & 61.67 +/- 2.85&  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> main/table/ablation_study_planning_horizon.tex <==
\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
%\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{Horizon=3} & \textbf{Horizon=6} & \textbf{Horizon=9} \\
\midrule
Medium-Expert-High & Hopper      &  56.73 +/- 3.48 & 60.65 +/- 3.49 &  71.26 +/- 3.98 \\
Medium-Expert-High & Walker2D    &  74.73 +/- 3.13 & 82.59 +/- 2.95 & 97.18 ± 2.08 \\
\midrule
Medium-High        & Hopper      & 50.09 +/- 3.29  & 51.14 +/- 3.39  &  55.32 ± 3.56\\
Medium-High        & Walker2D    &  62.08 +/- 2.20 &  66.63 +/- 2.74 & 68.87 ± 2.21\\
\midrule
Medium-Replay-High & Hopper      &  49.60 +/- 3.04 &  53.76 +/- 3.00 & 62.49 +/- 3.65\\
Medium-Replay-High & Walker2D    &  51.85 +/- 3.37  & 60.31 +/- 2.79  &  65.10 +/- 2.49\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


%57.51;62.51;70.04

==> main/table/ablation_study_progressive_widening.tex <==
\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
%\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{$\alpha$=0} & \textbf{$\alpha$=1} \\
\midrule
Medium-Expert-High & Hopper      &   & 62.78 +/- 3.47 &  51.33 +/- 3.26\\
Medium-Expert-High & Walker2D    &   & 98.47 +/- 3.11 &  89.56 +/- 2.98\\
\midrule
Medium-High        & Hopper      &   & 52.07 +/- 3.67  &  40.70 +/- 2.70\\
Medium-High        & Walker2D    &   & 67.62 +/- 2.05 &  57.85 +/- 2.73\\
\midrule
Medium-Replay-High & Hopper      &   & 49.68 +/- 3.06 &  35.60 +/- 2.53\\
Medium-Replay-High & Walker2D    &   & 64.22 +/- 2.79  & 47.59 +/- 3.52 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> main/table/ablation_study_records.tex <==
No ood:  54.10 +/- 3.18; 53.07 +/- 3.40; 54.10 +/- 3.18; 59.52 +/- 3.14; 68.86 +/- 2.31; 95.33 +/- 2.21
%64.16




==> main/table/relative_peformance_inference_time.tex <==
%pwd parameters: 0;0.1;0.2
%performance with cache tree, (pwd 0; pwd 0.1; pwd 0.2), mcts 50, 100, 200, decision time
%performance without cache tree, mcts 50, 100, 200, decision time

%mcts 200: 64.24 +/- 6.61
mcts 100:  62.40 +/- 5.50
0.30942186396172705 0.00010062415964508685
mcts 50:  57.04 +/- 5.77 
0.16047570644280848 4.6136718471850285e-05
mcts 10:    57.19 +/- 6.04 0.040267971538057265 6.530823670075905e-06




cache tree 100: 66.93 ± 3.46
0.09851784873427007 0.00028909328196628537
cache tree 50: 62.40 +/- 3.73
0.07152290527637188 3.052743115779859e-05
cache tree 10: 56.32 +/- 3.24
0.04593579292297363 1.1533768387016611e-05

==> main/table/sampling_deterministic_env.tex <==
% \begin{table}[]
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Dataset Type  & Env         & Sampling=1 & Sampling=4 & Sampling=8 \\ \hline
% Medium-Expert & HalfCheetah & 91.37 +/- 0.44  &  92.88 +/- 0.27  & 92.33 +/- 1.11   \\ \hline
% Medium-Expert & Hopper      & 102.21 +/- 4.56  &  104.09 +/- 4.25  &  110.93 +/- 2.00 \\ \hline
% Medium-Expert & Walker2D    & 109.44 +/- 0.11  & 109.66 +/- 0.16 & 109.75 +/- 0.11  \\ \hline
% Medium        & HalfCheetah &  43.80 +/- 0.23    &  44.75 +/- 0.27  &   44.42 +/- 0.36       \\ \hline
% Medium        & Hopper      &  79.02 +/- 3.63    & 80.48 +/- 3.83  &    86.26 +/- 1.93        \\ \hline
% Medium        & Walker2D    &  81.63 +/- 0.34    &  82.30 +/- 0.38  &  82.45 +/- 0.85  \\ \hline
% Medium-Replay & HalfCheetah & 36.75 +/- 0.98  &  36.99 +/- 0.68  &  38.37 +/- 0.39       \\ \hline
% Medium-Replay & Hopper      & 88.87 +/- 2.59  & 91.63 +/- 0.50  &  92.39 +/- 0.48  \\ \hline
% Medium-Replay & Walker2D    &  70.35 +/- 6.96  &   81.92 +/- 4.89  &   83.08 +/- 3.76  \\ \hline
% \end{tabular}
% \caption{Performance improvement caused by sampling in deterministic env, this table is evaluate with three model over 20 episodes.(Adding number of episodes right now )}
% \end{table}


\begin{table}[htbp]
\centering
\caption{Performance improvement caused by sampling in deterministic environments. This table evaluates three models over 20 episodes.}
\label{tab:sampling_results}
\begin{adjustbox}{width=0.7\textwidth}
\begin{tabular}{llccc}
\toprule
\textbf{Dataset Type} & \textbf{Env} & \textbf{Sampling=1} & \textbf{Sampling=4} & \textbf{Sampling=8} \\
\midrule
Medium-Expert & HalfCheetah & 91.37 $\pm$ 0.44  & \textbf{92.88 $\pm$ 0.27}  & 92.33 $\pm$ 1.11 \\
Medium-Expert & Hopper      & 102.21 $\pm$ 4.56 & 104.09 $\pm$ 4.25 & \textbf{110.93 $\pm$ 2.00} \\
Medium-Expert & Walker2D    & 109.44 $\pm$ 0.11 & 109.66 $\pm$ 0.16 & \textbf{109.75 $\pm$ 0.11} \\
\midrule
Medium        & HalfCheetah & 43.80 $\pm$ 0.23  & \textbf{44.75 $\pm$ 0.27}  & 44.42 $\pm$ 0.36 \\
Medium        & Hopper      & 79.02 $\pm$ 3.63  & 80.48 $\pm$ 3.83  & \textbf{86.26 $\pm$ 1.93} \\
Medium        & Walker2D    & 81.63 $\pm$ 0.34  & 82.30 $\pm$ 0.38  & \textbf{82.45 $\pm$ 0.85} \\
\midrule
Medium-Replay & HalfCheetah & 36.75 $\pm$ 0.98  & 36.99 $\pm$ 0.68  & \textbf{38.37 $\pm$ 0.39} \\
Medium-Replay & Hopper      & 88.87 $\pm$ 2.59  & 91.63 $\pm$ 0.50  & \textbf{92.39 $\pm$ 0.48} \\
Medium-Replay & Walker2D    & 70.35 $\pm$ 6.96  & 81.92 $\pm$ 4.89  & \textbf{83.08 $\pm$ 3.76} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

%78.16;80.52;82.22 for all results
%88.59;91.68;94.14 for results exclude halfcheetah

==> main/table/standard_VAE_loss.tex <==
%hopper high medium expert: 52.41 +/- 3.19
%hopper high medium :  44.82 +/- 3.27 
%hopper high medium replay: 43.69 +/- 2.60
%walker2d high medium expert: 88.21 +/- 2.42 
%walker2d high medium : 58.33 +/- 2.12
%walker2d high medium replay: 56.10 +/- 3.31
